Conformations, correlations, and instabilities of a flexible fiber in an active fluid

Fluid-structure interactions between active and passive components are important for many biological systems to function. A particular example is chromatin in the cell nucleus, where ATP-powered processes drive coherent motions of the chromatin fiber over micron lengths. Motivated by this system, we develop a multiscale model of a long flexible polymer immersed in a suspension of active force dipoles as an analog to a chromatin fiber in an active fluid -- the nucleoplasm. Linear analysis identifies an orientational instability driven by hydrodynamic and alignment interactions between the fiber and the suspension, and numerical simulations show activity can drive coherent motions and structured conformations. These results demonstrate how active and passive components, connected through fluid-structure interactions, can generate coherent structures and self-organize on large scales.

==> commands.tex <==


\let\caron\v
\let\cedilla\c

\usepackage{amsmath,amsfonts,amssymb,bm,dsfont,mathtools,xcolor}
\usepackage{graphicx,scrextend}
\usepackage{enumerate}

\DeclarePairedDelimiter{\set}{\{}{\}}
\DeclarePairedDelimiter{\bpar}{\Big (}{\Big )}
\DeclarePairedDelimiter{\babs}{\Big |}{\Big |}
\DeclarePairedDelimiter{\bbrack}{\Big [}{\Big ]}
\DeclarePairedDelimiter{\norm}{|\!|}{|\!|}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\trace}{tr}
\DeclarePairedDelimiter{\lr}{\langle}{\rangle}

\newcommand{\ints}{\int\limits}
\newcommand{\lims}{\lim\limits}
\newcommand{\sums}{\sum\limits}
\renewcommand{\Im}{\text{Im}}
\newcommand{\eps}{\varepsilon}
\newcommand{\grad}{\nabla}
\renewcommand{\div}{\nabla\cdot}

\renewcommand{\a}{\mathbf{a}}
\renewcommand{\b}{\mathbf{b}}
\renewcommand{\c}{\mathbf{c}}
\renewcommand{\d}{\mathbf{d}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\f}{\mathbf{f}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\h}{\mathbf{h}}
\renewcommand{\k}{\mathbf{k}}
\newcommand{\m}{\mathbf{m}}
\newcommand{\n}{\mathbf{n}}
\newcommand{\p}{\mathbf{p}}
\newcommand{\q}{\mathbf{q}}
\renewcommand{\r}{\mathbf{r}}
\newcommand{\s}{\mathbf{s}}
\renewcommand{\t}{\mathbf{t}}
\renewcommand{\u}{\mathbf{u}}
\renewcommand{\v}{\mathbf{v}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\z}{\mathbf{z}}

\newcommand{\hk}{\hat\k}
\newcommand{\hz}{\hat\z}


\newcommand{\ta}{\tilde{\mathbf{a}}}
\newcommand{\tb}{\tilde{\mathbf{b}}}
\newcommand{\tc}{\tilde{\mathbf{c}}}
\newcommand{\td}{\tilde{\mathbf{d}}}
\newcommand{\te}{\tilde{\mathbf{e}}}
\newcommand{\tf}{\tilde{\mathbf{f}}}
\newcommand{\tk}{\tilde{\mathbf{k}}}
\newcommand{\tm}{\tilde{\mathbf{m}}}
\newcommand{\tn}{\tilde{\mathbf{n}}}
\newcommand{\tp}{\tilde{\mathbf{p}}}
\newcommand{\tq}{\tilde{\mathbf{q}}}
\newcommand{\tu}{\tilde{\mathbf{u}}}
\newcommand{\tv}{\tilde{\mathbf{v}}}
\newcommand{\tx}{\tilde{\mathbf{x}}}
\newcommand{\tz}{\tilde{\mathbf{z}}}

\newcommand{\hs}{\hat{\mathbf{s}}}

\newcommand{\tphi}{\tilde\phi}
\newcommand{\ttau}{\tilde\btau}


\newcommand{\A}{\mathbf{A}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\C}{\mathbf{C}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\E}{\mathbf{E}}
\newcommand{\F}{\mathbf{F}}
\newcommand{\G}{\mathbf{G}}
\renewcommand{\H}{\mathbf{H}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\R}{\mathbf{R}}
\renewcommand{\S}{\mathbf{S}}
\newcommand{\T}{\mathbf{T}}
\newcommand{\U}{\mathbf{U}}
\newcommand{\V}{\mathbf{V}}
\newcommand{\X}{\mathbf{X}}

\newcommand{\tA}{\tilde{\mathbf{A}}}
\newcommand{\tB}{\tilde{\mathbf{B}}}
\newcommand{\tC}{\tilde{\mathbf{C}}}
\newcommand{\tD}{\tilde{\mathbf{D}}}
\newcommand{\tE}{\tilde{\mathbf{E}}}
\newcommand{\tF}{\tilde{\mathbf{F}}}
\newcommand{\tG}{\tilde{\mathbf{G}}}
\newcommand{\tM}{\tilde{\mathbf{M}}}
\newcommand{\tI}{\tilde{\mathbf{I}}}
\newcommand{\tQ}{\tilde{\mathbf{Q}}}
\newcommand{\tR}{\tilde{\mathbf{R}}}
\newcommand{\tS}{\tilde{\mathbf{S}}}
\newcommand{\tT}{\tilde{\mathbf{T}}}
\newcommand{\tU}{\tilde{\mathbf{U}}}
\newcommand{\tV}{\tilde{\mathbf{V}}}
\newcommand{\tX}{\tilde{\mathbf{X}}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}


\newcommand{\btau}{\bm\tau}
\newcommand{\bLambda}{\bm\Lambda}
\newcommand{\bOmega}{\bm\Omega}
\newcommand{\bSigma}{\bm\Sigma}
\newcommand{\tSigma}{\tilde\bSigma}

\renewcommand{\L}{\mathcal L}

